A Formal Model for Artificial Intelligence Applications in Automation Systems

The integration of Artificial Intelligence (AI) into automation systems has the potential to enhance efficiency and to address currently unsolved existing technical challenges. However, the industry-wide adoption of AI is hindered by the lack of standardized documentation for the complex compositions of automation systems, AI software, production hardware, and their interdependencies. This paper proposes a formal model using standards and ontologies to provide clear and structured documentation of AI applications in automation systems. The proposed information model for artificial intelligence in automation systems (AIAS) utilizes ontology design patterns to map and link various aspects of automation systems and AI software. Validated through a practical example, the model demonstrates its effectiveness in improving documentation practices and aiding the sustainable implementation of AI in industrial settings.

==> archive/04_related_work.tex <==
\section{Related Works} \label{sec:related_works}
We identified three areas of relevant research: data sheets, ontologies and graphical modeling. The most relevant works in the respective areas are briefly presented in the following:

\subsection{Sheets and Cards}
One area of research focuses on creating \textit{sheets} and \textit{cards} (S\&C), which are short documents with predefined categories to  capture relevant information about the AI application. In order to obtain the relevant information, the authors use a number of predefined questions that must be answered by the developers of the AI application.

For example, \citet{gebru2018} proposed a approach called \textit{Datasheets for Datasets} to reflect and document the creation process, distribution, maintaining and assumptions as well as the risks and implications of a used dataset. The Questions for creating the datasheets depend on the organizational infrastructure and the used workflow.

Inspired by Datasheets for Datasets the authors \citet{mitchell2019} proposed a framework called \textit{Model Cards} to encourage transparent model reporting. Model cards are an extension to data sheets for data sets, but for AI models. Model Cards are short documents for trained machine learning models to provide benchmarks of the model performance in different conditions. The focus is on trained model characteristics and model details like type of model used, intended use case, metrics used, evaluation data used, training data used and performance variation.

\citet{arnold2019} proposes \textit{FactSheets} to increase trust in AI-Services by documenting various characteristics of AI services, including whether the data used to develop the services are accompanied by datasheets. FactSheets are documents that contain sections on several relevant attributes of an AI service, such as intended use, performance, safety, and security, as well as data and evaluation information. In this way, FactSheets are somehow a combination of model-cards and datasheets. In order to obtain the relevant information, the authors have created a number of questions that must be answered for each data set used by the developers. 

\citet{lavin2022} proposes a framework for \textit{Machine Learning Technology Readiness Levels} (MLTRL) that defines a process for ensuring robust, reliable and responsible ML systems and an approach for documenting the TLR level through so-called \textit{Technology-Readiness-Level-Cards} (TLR-Cards). The content of a TLR-Cards can be divided into the categories: project info and implicit knowledge. Project info clearly states information such as project owners and reviewers, development status, and semantic versioning just for code, for models and for data. These information are very similar to that contained in Datasheets, Model Cards and FactSheets. The implicit knowledge documents more specific insights gained throughout the development process that need to be communicated to the stakeholders like modeling assumptions, dataset biases and corner cases.

\subsection{Ontologies}
A second area of research focuses on documenting AI applications in a more formal way by using ontologies instead of sheets and cards \cite{sinha2022dm, sinha2021ml}. These formal and ontology-based approaches are used as a basis for large community platforms like OpenML \cite{vanschoren2014}. 
Within this research area, one group focuses on ontologies to support the creation and documentation of the underlying development process.

For example, \citet{panov2013} propose an ontology called OntoDM-KDD for representing the knowledge discovery process based on the \textit{Cross Industry Standard Process for Data Mining} (CRISP-DM). The ontology aims to be general enough to allow the representation of knowledge discovery processes based on CRISP-DM in practical applications. At the highest level, this ontology consists of the process steps of CRISP-DM. These steps are then successively detailed in order to capture ever more precise information and correlations of the development process. Furthermore, \citet{panov2014} proposes a second ontology called OntoDM, wich is a more general approach than OntoDM-KDD and not limited to a specific workflow or process, such as CRISP-DM. OntoDM provides a representational framework for the description of mining structured data, and in addition provides taxonomies of datasets, data mining tasks, generalizations, data mining algorithms and constraints, based on the type of data.

\citet{keet2015} proposed an ontology called \textit{Data Mining Optimization Ontology} (DMOP) to simplify the decision-making within a data mining process and to optimize the performance of DM processes. DMOP provide a unified conceptual framework for analyzing DM tasks, algorithms, models, datasets, workflows and performance metrics, and their relationships. Furthermore, the ontology is not limited to a specific workflow, such as CRISP-DM.

Within the research area of ontologies, a second group focuses on ontologies that support the documentation of models and algorithms, especially for machine learning \cite{sinha2021ml}.
%Expose
For example, the purpose of the ontology proposed by \citet{vanschoren2010} is to model the ML experimentation called \textit{Exposé}. The ontology represents a formal domain model that can properly elucidate the different experiments performed in ML. The main elements are information about the mining experiments, details of the used algorithms and the used datasets.
%MEX
\citet{esteves2015} proposed an ontology which purpose is to describe the provenance information for machine learning experiments called \textit{MEX Vocabulary}. 
%MLSchema
\citet{publio2018} proposes an ontology for representing and interchanging information on machine learning algorithms, datasets and experiments called \textit{ML-Schema}. It is maintained by the W3C ML-Schema Community Group\footnote{https://www.w3.org/community/ml-schema/}.

\subsection{Graphical Modeling}
A graphical model can be used to represent the core of a problem in a semiformal and understandable way for different stakeholders and experts. The overarching goal of graphical modeling is to represent the task and solution of the problem as formally as possible and thus facilitate the solution finding and communication of all actors involved in the development and to document the solution in a graphical representation. \cite{schnieder1999}

An approach specifically for the graphical representation of AI systems was presented by \Citet{kaymakci2021}, which is based on the representation of data sources, data sinks and data-processing elements. On this basis, a graphical modeling language was proposed by \citet{schieseck2023} which can represent AI systems within automation systems. It is based on the systems engineering theory of \citet{haberfellner2019} and therefore describes the entire system with three main element types: 1.) system components, 2.) system functions and 3.) system relations. The system relations, such as communication, assignment, and product flow, relate the elements to each other. The authors defined a symbolism and a syntax to represent and interrelate the graphical elements. In addition, they provide a metamodel\footnote{https://github.com/schiesem/GML-AIAAS} for further formalization.

\subsection{Discussion of Related Works}
After presenting the relevant areas and related works, a discussion and evaluation are conducted based on the presented requirements.

% Cards and Sheets
The cards and sheets only allow a description of the AI components and the data. Documenting the technical system, the technical process as well its interdependencies is not included and not intended by the authors (R1). Even though the C\&S itself are divided into predefined categories and the information are gathered due to predefined questions, the answers are mainly given in free text form (R3). As a result, the formality and accuracy relies on the integrity and experience of the person, who answers the questions \cite{mitchell2019}. The C\&S are not specified to the vocabulary of a vendor or a programming language, but also not to standards or legislations (R2). Due to the simple structure, they can be easily expanded and adapted to different use cases or domains (R4).
% Ontologies 
The approaches based on ontologies are, by their very nature, completely formalized (R3). Most of the approaches are using OWL\footnote{https://www.w3.org/OWL/} as vendor-independent format (R2). Neither the ontologies focussing on data mining processes nor those focussing on ML algorithms and models allow the consideration of the technical process, the technical system their interdependencies to the AI components (R1). Furthermore, the ontologies are not built up on standards or regulations or reference them (R2). In addition, most of the ontologies are not semantically consistent or aligned with each other. Most of the presented ontologies are large, monolithic blocks consisting of many classes and relationships. Even if these ontologies are easy to expand and adapt in principle, in reality it is still difficult due to the large, monolithic structure (R4).
% Further Approaches
Besides the approaches using sheets and cards or ontologies, also approaches using graphical modeling were presented. In its core, the approach of \citet{schieseck2023} allows the representation of interdependencies between technical system, technical process and AI functions (R1) through a defined symbolism and syntax. By additionally using the provided metamodel, the symbolism can be transformed and formalized in a vendor-neutral format (R3), e.g. XML or JSON. No vendor- or programming language-specific terms are used, but also no semantic references are made to standards or legislations (R2). Due to the simple structure of the metamodel, the content can be easily expanded and adapted (R4).

In summary, none of the existing approaches is able to fulfill the requirements and therefore is able to solve the existing problem. There is a lack ... Therefore, a new approach is needed, which is presented in the following.

==> archive/validation_example.tex <==
\subsubsection*{Modeling the Application Example}
Following the presented modeling principle, the information of the application example successively need to be instantiated and connected using the respective classes. 
For the given use-case, the input product of the technical process is a metal plate. This can exemplary be models as follows: An instance of the class \texttt{AIAS:Process} is created and named \texttt{ex:stampingProcess}. Then the class \texttt{VDI3682:Product} is used to create an instance named \texttt{ex:rawMetalPlate}, describing the input product. Afterward, an instances of the class \texttt{VDI3682:Flow} is created, named \texttt{ex:stampingInputFlow}. Firstly, \texttt{AIAS:hasProcess} is used connect the instance \texttt{ex:stampingInputFlow} with the process \texttt{ex:stampingProcess}. Afterward, with the help of \texttt{AIAS:hasProduct} the instance  \texttt{ex:stampingInputFlow} is linked to \texttt{ex:rawMaterial}. The output of the process could also be modeled in the same way.

In the given use-case, there are several communications, for example between the edge device and the cloud. This can exemplary be models as follows: An instance of the class \texttt{AIAS:EdgeDevice} named \texttt{ex:RaspberryPi} and an instance of the class \texttt{AIAS:Cloud} named \texttt{ex:Azure} are created. Then the class \texttt{ISO7489:Communication} is used to create \texttt{ex:Ethernet1}. Using the subclasses of the ISO7489 ODP, the \texttt{Ethernet1} could be specified in detail using for example the \texttt{ISO7489:hasLayer}, \texttt{ISO7489:Layer} and \texttt{ISO7489:Technology} classes. With the help of \texttt{AIAS:hasCommunication}, the instances \texttt{ex:RaspberryPi} and \texttt{ex:EdgeDevice} can be connected to \texttt{ex:Ethernet1} and thus define the communication. 

In the given use-case, the training was done in the cloud and the inference is deployed on the edge device. This can exemplary be modeled using assignments as follows: An instance of the class \texttt{ISO22989:Train} called \texttt{ex:networkTraining} and an instance of \texttt{}
